Improving Examples in Web API Specifications using Iterated-Calls In-Context Learning

Examples in web API specifications can be essential for API testing, API understanding, and even building chat-bots for APIs. Unfortunately, most API specifications lack human-written examples. This paper introduces a novel technique for generating examples for web API specifications. We start from in-context learning (ICL): given an API parameter, use a prompt context containing a few examples from other similar API parameters to call a model to generate new examples. However, while ICL tends to generate correct examples, those lack diversity, which is also important for most downstream tasks. Therefore, we extend the technique to iterated-calls ICL (ICICL): use a few different prompt contexts, each containing a few examples,to iteratively call the model with each context. Our intrinsic evaluation demonstrates that ICICL improves both correctness and diversity of generated examples. More importantly, our extrinsic evaluation demonstrates that those generated examples significantly improve the performance of downstream tasks of testing, understanding, and chat-bots for APIs.

==> Makefile <==
# Set this to the basename of the .tex file
# This will also be the name of the generated .dvi, .ps and .pdf files

.PHONY: paper all clean

# Set this to the other source files that should be counted as
# dependencies
OTHERSOURCES := bibliography.bib \
	acmart.bib \
	$(filter-out main.tex, $(wildcard *.tex))

all: paper

PDFLATEX = pdflatex -synctex=1 --shell-escape
BIBTEX = bibtex
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

paper: main.pdf

tidy:
	rm -rf *.aux *.out *.bbl *.toc *.log *.blg *.pyg *.cpt _minted*

# Using latexmk to generate the PDF
%.pdf: %.tex $(OTHERSOURCES)
	${PDFLATEX} $<; ${PDFLATEX} $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(PDFLATEX) $<;$(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep -i "(Reference|Citation).*undefined" $*.log ; true

clean: tidy
	@\rm -f \
        *.{aux,log,out,dvi,ps,bbl,blg} \
        *.{gnuplot,fdb_latexmk,fls,upa,upb,cut} \
	main.pdf


==> dataavailability.tex <==
\section{Data Availability}

We make \technique's code, intrinsic evaluation, fuzzing evaluation, and exploratory study publicly available at \url{https://figshare.com/s/8eec881ddf8e6573f43f}. 
The README file documents steps to reproduce our results.
We are not able to release our API parameter bank, intrinsic evaluation dataset, and SeqATIS dataset due to employer restrictions. 

